SheetCopilot: Bringing Software Productivity to the Next Level through Large Language Models

Computer end users have spent billions of hours completing daily tasks like tabular data processing and project timeline scheduling. Most of these tasks are repetitive and error-prone, yet most end users lack the skill to automate these burdensome works. With the advent of large language models (LLMs), directing software with natural language user requests become a reachable goal. In this work, we propose a SheetCopilot agent that takes natural language task and control spreadsheet to fulfill the requirements. We propose a set of atomic actions as an abstraction of spreadsheet software functionalities. We further design a state machine-based task planning framework for LLMs to robustly interact with spreadsheets. We curate a representative dataset containing 221 spreadsheet control tasks and establish a fully automated evaluation pipeline for rigorously benchmarking the ability of LLMs in software control tasks. Our SheetCopilot correctly completes 44.3\% of tasks for a single generation, outperforming the strong code generation baseline by a wide margin. Our project page:https://sheetcopilot.github.io/.

==> figure/AblationsRadarCharts.tex <==
% 单图
% \begin{figure}
%     \centering
%     \begin{tikzpicture}
%     \begin{polaraxis}[
%         yticklabels={},
%         xticklabel style={anchor=-22.5},
%         xtick={0,45,90,135,180,225,270,315},
%         xticklabels={Variable 1, Variable 2, Variable 3, Variable 4},
%         grid=both,
%         major grid style={line width=0.2pt,draw=gray!50},
%         width=0.6\textwidth,
%         height=0.6\textwidth
%     ]
    
%     \addplot[fill=blue!30, opacity=0.7] coordinates {
%         (0,0)
%         (45,0.4)
%         (90,0.7)
%         (135,0.9)
%     };
    
%     \end{polaraxis}
%     \end{tikzpicture}
%     \caption{Radar Chart}
% \end{figure}


% 多图
\begin{figure}
    \centering    
    \begin{subfigure}[b]{0.3\textwidth}
             \centering
             \includegraphics[scale=0.185]{figure/Comparisono_by_Category.png}
             \label{fig: ablation on closedloop}
             \caption{}
             \label{subfig:countryA}
         \end{subfigure}
    \hfill
         \begin{subfigure}[b]{0.3\textwidth}
             \centering
            \includegraphics[scale=0.185]{figure/Comparisono_by_Category.png}
            \label{fig: ablation on doc}
                \caption{}
             \label{subfig:countryB}
         \end{subfigure}
    
    \caption{\textbf{The ablation results of closed-loop control (a) and external document insertion (b) on the six categories}}
\end{figure}

==> figure/chat_dialogue_example.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{figure/chat_dialogue_example.png}
  \caption{The chat dialogue figure.}
  \label{fig:chat_dialogue}
\end{figure}

==> table/Experiments/AblateLoopDoc.tex <==
\begin{table}[ht]
    \scriptsize
    \centering
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \caption{Ablation study of closed-loop control. Compared with the open loop variant, the two types of feedback increase the Exec@1 and Pass@1 when individually applied and bring a significant improvement when both are applied.}
            \label{tab: ablate closed-loop}
            \begin{tabular}{@{}ccccc@{}}
            \toprule
            Models                           & Exec@1 & Pass@1 & A50 & Q50 \\ \midrule
            Plain                            & 56.6\%   & 25.8\%    & 3  &  4   \\ % output_dataset_515_plain
            Open loop                        & 67.8\%   & 28.1\%   &  2  &  7   \\ % NoFeedBack_T_0
            + sheet state feedback           & 76.0\%   & 36.2\% &  3  & 8 \\ 
            + error feedback                 & 79.1\%   & 39.3\%   &  3  &  7   \\ % output_dataset_514_no_state
            Ours full                        & 87.3\% &  44.3\%  &  4  & 9   \\  % human verification by Jingran
            % Ours full跑了两轮 &   73.8 + 75.6   &  40.3 + 42.5 &  3 + 4 & 9 + 9 & 5.2 + 5.7 & 13.0 + 13.0 \\  % Round1_T_0 + Round2_T_0

            \bottomrule
            \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.49\linewidth}
        \centering
            \caption{Ablation study of external document insertion. }
            \label{tab: ablate doc insertion}
            \begin{tabular}{@{}ccccc@{}}
            \toprule
            Detailedness of API & Exec@1 & Pass@1 & A50 & Q50 \\ 
            \midrule
            Plain                            & 56.6\%   & 25.8\%    & 3  &  4   \\ % output_dataset_515_plain
            -doc -example &  68.3\%  &  25.8\%  &  3  &  4      \\ % output_dataset_514_no_doc_no_example
            +doc -example &  86.0\%  & 43.9\%   &  3  & 8    \\ % NoExample_T_0
            +doc +example (Ours full) & 87.3\% &  44.3\%  &  4  & 9      \\ 
            \bottomrule
            \end{tabular}
    \end{minipage}
\end{table}

==> table/Experiments/ComparisonWithVBA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
\caption{Comparison with VBA.}
\label{tab: vba}
\begin{tabular}{@{}c|cc@{}}
\toprule
Models        & Exec@1 & Pass@1  \\ 
\midrule
Ours & 87.3\% &  44.3\%   \\ 
VBA  & 77.8\%  & 37.1\%    \\

\bottomrule

\end{tabular}
\end{table}

==> table/Experiments/Stability.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table}[tp]
\footnotesize
\centering
\caption{Stability test. Row 1 records the result of running our method once at temperature = 0.0. Row 2 records the average of the results of running our method 3 times at temperature = 0.2. }
\label{tab: stability test}
\begin{tabular}{@{}c|cccccc@{}}
\toprule
Temperature        & Exec@1$\uparrow$ & Pass@1$\uparrow$ & A50$\downarrow$ & A90$\downarrow$ \\ 
\midrule
0.0   & 87.3\%      & 44.3\%        & 1.50        & 3.00        \\
0.2  & 91.9\% &  44.6\% & 1.47 & 3.50 \\ 
% 0.2  & 91.9\% (4.6\%) &  44.6\% (0.5\%) & 1.47 (0.05) & 3.50 (0.00) \\ 
% 0.2 & GPT-3.5-Turbo &  97.3, 92.3, 86.0 &  44.8, 45.2, 43.9 & 1.40, 1.50, 1.50 & 3.50, 3.50, 3.50
\bottomrule

\end{tabular}
\end{table}


% 旧版指标
% \begin{table}[]
% \footnotesize
% \centering
% \caption{Stability test. Row 1 records the result of running our method once at temperature = 0.0. Row 2 records the result of running our method 3 times at temperature = 0.2. }
% \label{tab: stability test}
% \begin{tabular}{@{}cc|cccccc@{}}
% \toprule
% Temperature & Models        & Executable@1  & Pass@1 & A50 & Q50 & A90 & Q90 \\ 
% \midrule
% 0.0  & GPT-3.5-Turbo & 87.3\% & 44.3\% & 4.0   & 9.0  & 8.0 & 13.0 \\
% 0.2 & GPT-3.5-Turbo & 91.9\% (4.6) &  44.6\% (0.5) & 4.0 (0.0) & 9.0 (0.0) & 9.2 (0.3) & 13.0 (0.0) \\ 
% % 0.2 & GPT-3.5-Turbo &  97.3, 92.3, 86.0 &  44.8, 45.2, 43.9 & 4, 4, 4 & 9, 9, 9 & 9.0, 9.1, 9.4 & 13.0, 13.0, 13.0\\ 
% \bottomrule

% \end{tabular}
% \end{table}

==> text/3-eval.tex <==
\section{Eval}
We develop an automated, reproducible evaluation framework closely tailored to our curated natural language spreadsheet control dataset. 
This enables systematically assessing model abilities, gaining insights into current limitations, and driving continued progress in this domain.

\subsection{Task Evaluation by Execution}
We cannot evaluate proposed task solutions through verbatim comparison, as there are multiple solutions that could successfully complete a task.  
A viable approach is assessing whether executing the solution meets the task instruction.
We only assess necessary properties required for the ground truth spreadsheet's operation. 
For example, in the task "Plot a line chart with the X-axis showing the week and the Y-axis showing sales", we only consider properties related to the chart, ignoring other aspects.
We evaluate consistency of necessary properties between the spreadsheet resulting from executing the LLM generated plan in our simulation environment and the ground truth spreadsheet.
If the necessary properties of the resulting spreadsheet fully match any potential ground truth candidates, we deem the associated solution correct.

% In order to evaluate the plan, we compare the difference between the result spreadsheet produced by executing the proposed plan in the simulation environment and the ground truth spreadsheet.

\subsection{Simulation Environment}
The simulation environment serves as a crucial element of our evaluation framework, as it facilitates the interaction between LLMs and spreadsheets.  It controls the spreadsheet application to execute the plans generated by the LLMs, ensuring that the intended tasks are performed accurately and efficiently.
% Our simulation environment establishes the interaction between LLMs and spreadsheets, which controls the spreadsheet application to execute the planning generated by LLMs.
% By providing a controlled environment, we can effectively measure the model's performance, identify areas for improvement, and ensure that the generated planning are executed correctly.
Specifically, the simulation environment incorporates 21 atomic actions that cover the majority of spreadsheet operations. On one hand, simulation environment manipulate target spreadsheets using atomic actions based on the plan; on the other hand, it provides real-time feedback on the current execution results.

The simulation environment is designed to be flexible and adaptable, allowing it to work with a wide range of spreadsheet applications. In our experiment, we have implemented a backend that interfaces with Microsoft Excel 2016 using pywin32 library ~\cite{}, which enables access to the Windows operating system and its applications.

\yuntao{Jingran add more details about the env}
\yuntao{Give a general description, do not limit the spreadsheet to Excel}

